Commit Messages in the Age of Large Language Models

Commit messages are explanations of changes made to a codebase that are stored in version control systems. They help developers understand the codebase as it evolves. However, writing commit messages can be tedious and inconsistent among developers. To address this issue, researchers have tried using different methods to automatically generate commit messages, including rule-based, retrieval-based, and learning-based approaches. Advances in large language models offer new possibilities for generating commit messages. In this study, we evaluate the performance of OpenAI's ChatGPT for generating commit messages based on code changes. We compare the results obtained with ChatGPT to previous automatic commit message generation methods that have been trained specifically on commit data. Our goal is to assess the extent to which large pre-trained language models can generate commit messages that are both quantitatively and qualitatively acceptable. We found that ChatGPT was able to outperform previous Automatic Commit Message Generation (ACMG) methods by orders of magnitude, and that, generally, the messages it generates are both accurate and of high-quality. We also provide insights, and a categorization, for the cases where it fails.

==> todo.tex <==
\paragraph{\textbf{Implications for testers}}
In our work, we identified ASP can generate divergent test examples with a few subordinate prefixes and effectively find the bugs that a conversational agent has. By incorporating the ASP approach, the testers can easily find the bugs in a system with little manual work. In addition, ASP-identified sources of weaknesses can be utilized by testers while debugging and curating the dataset used for evaluating the conversational agents.

\paragraph{\textbf{Implications for researchers}}
In our work, we proposed a new example generation methodology that shows great effectiveness and efficiency in testing an airline conversational system. This study can be expanded to test conversational agents in various domains. We encourage researchers to examine the generalizability of our testing approach. Furthermore, our results demonstrated that general context subordinate prefixes also could identify bugs in the system. Further research could involve creating a large database of general context subordinate prefixes that can be used for testing any conversational agent. Researchers should also investigate automated ways of augmenting the data while using the weaknesses identified by ASP as the guiding mechanism.

\paragraph{\textbf{Implications for tool builders}}
When building a conversational system, it is as important to provide an evaluation of the system as it is to build a good system by training the data well. ASP can be added to a conversational agent builder IDE to provide the users with the performance of their systems. Secondly, we identified the sources of the weaknesses in a system from the analysis of prediction results with ASP. Finally, adding analytic technologies to the IDE can offer the user valuable insights, enabling them to enhance the system by enriching data, modifying existing data, and more.
